I Know What You Trained Last Summer: A Survey on Stealing Machine Learning Models and Defences

Machine Learning-as-a-Service (MLaaS) has become a widespread paradigm, making even the most complex machine learning models available for clients via e.g. a pay-per-query principle. This allows users to avoid time-consuming processes of data collection, hyperparameter tuning, and model training. However, by giving their customers access to the (predictions of their) models, MLaaS providers endanger their intellectual property, such as sensitive training data, optimised hyperparameters, or learned model parameters. Adversaries can create a copy of the model with (almost) identical behavior using the the prediction labels only. While many variants of this attack have been described, only scattered defence strategies have been proposed, addressing isolated threats. This raises the necessity for a thorough systematisation of the field of model stealing, to arrive at a comprehensive understanding why these attacks are successful, and how they could be holistically defended against. We address this by categorising and comparing model stealing attacks, assessing their performance, and exploring corresponding defence techniques in different settings. We propose a taxonomy for attack and defence approaches, and provide guidelines on how to select the right attack or defence strategy based on the goal and available resources. Finally, we analyse which defences are rendered less effective by current attack strategies.

==> tab-comparison-old.tex <==
{
\setlength{\tabcolsep}{1pt}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}

\begin{tabular}{
|p{2.77cm} % first col
|C{0.90cm}|C{1.05cm}|C{1.05cm} % basic --
|C{1.40cm}|C{1.40cm}|C{1.08cm} % mod mod distill --
|C{0.99cm}|C{0.98cm}|C{0.89cm} % wm (dawn) --
|C{1.38cm}|C{1.38cm}|C{1.0cm} % out pert + mon --
|C{1.30cm}| % monitor + dp
% *{13}{|p{1.15cm}}|
}


\hline
Attack Types / Defence                                                                              & Basic \tiny{(top-1)} \tiny{\cite{tramer_stealing_2016}}                                                            & Monitor \tiny{\cite{kesarwani_model_2018}}              & Monitor \tiny{(PRADA)} \tiny{\cite{juuti_prada_2019}}   & Model mod. \tiny{(distill.)} \tiny{\cite{xu_deepobfuscation_2018}} & Model mod. \tiny{(parasatic)} \tiny{\cite{chabanne_protection_2020}} & No trans- fer \tiny{\cite{krishna_thieves_2020, atli_extraction_2020}} & WM  \tiny{(DAWN)} \tiny{\cite{szyller_dawn_2021}} & Input pert. \tiny{\cite{guiga_neural_2020}} & Output pert. \tiny{\cite{lee_defending_2019}}                 & Output pert. + monit. \tiny{\cite{kariyappa_defending_2020}} & Output pert.  \tiny{(MAD)} \tiny{\cite{orekondy_prediction_2020}} & DP \tiny{(BDPL)} \tiny{\cite{zheng_bdpl_2019}}  & Monitor + DP \tiny{(MDP)} \tiny{\cite{yan_monitoring-based_2021}} \\ \hline
Witn. Finding \tiny{\cite{lowd_adversarial_2005, tramer_stealing_2016, reith_efficiently_2019}}     &                                                                                                     &                                                         &                                                         &                                                                    &                                                                      &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  & \attackMitigatedMark {\tiny \cite{zheng_bdpl_2019}}           &                                                                   \\ \hline
ESA-P \tiny{\cite{tramer_stealing_2016, reith_efficiently_2019}}                                    & \defenceBrokenMark {\tiny \cite{tramer_stealing_2016}}  \defenceBrokenMark {\tiny \cite{reith_efficiently_2019}} \attackClaimMark &                                                         &                                                         &                                                                    &                                                                      &                                                                       &                                                   & \attackMitigatedMark {\tiny \cite{guiga_neural_2020}}    &                                                              &                                                              &                                                                  &                                                 & \attackMitigatedMark {\tiny \cite{yan_monitoring-based_2021}}                   \\ \hline
ESA-P \tiny{(dupl. quer.)} \tiny{\cite{yan_monitoring-based_2021}}                                  & \defenceBrokenMark {\tiny \cite{yan_monitoring-based_2021}}                                                     & \attackLoweredMark {\tiny \cite{yan_monitoring-based_2021}}    &                                                         &                                                                    &                                                                      &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  & \defenceBrokenMark {\tiny \cite{yan_monitoring-based_2021}} & \attackMitigatedMark {\tiny \cite{yan_monitoring-based_2021}}                   \\ \hline
PFA \tiny{\cite{tramer_stealing_2016}}                                                              & \defenceBrokenMark {\tiny \cite{tramer_stealing_2016}}                                                          & \attackMitigatedMark {\tiny \cite{kesarwani_model_2018}}              &                                                         &                                                                    &                                                                      &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  &                                                 &                                                                   \\ \hline
Recovery \tiny{\cite{jagielski_high_2020}}                                                          &                                                                                                     &                                                         &                                                         &                                                                    & \attackMitigatedMark {\tiny \cite{chabanne_protection_2020}} \attackClaimMark            &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  &                                                 &                                                                   \\ \hline
Recovery \tiny{\cite{rolnick_reverse-engineering_2020}}                                             &                                                                                                     &                                                         &                                                         &                                                                    & \attackMitigatedMark {\tiny \cite{chabanne_protection_2020}} \attackClaimMark            &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  &                                                 &                                                                   \\ \hline
Recovery \tiny{\cite{carlini_cryptanalytic_2020}}                                                   &                                                                                                     &                                                         &                                                         &                                                                    & \attackMitigatedMark {\tiny \cite{chabanne_protection_2020}} \attackClaimMark            &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  &                                                 &                                                                   \\ \hline
SMA-* \tiny{(retraining)} \tiny{\cite{tramer_stealing_2016, reith_efficiently_2019}}                &                                                                                                     &                                                         & \attackMitigatedMark {\tiny \cite{juuti_prada_2019}}                  &                                                                    &                                                                      &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  & \attackMitigatedMark {\tiny \cite{zheng_bdpl_2019}}           &                                                                   \\ \hline
SMA-\tiny{NN} \tiny{\cite{papernot_practical_2017}}                                                 &                                                                                                     &                                                         & \attackMitigatedMark {\tiny \cite{juuti_prada_2019}}                  &                                                                    &                                                                      &                                                                       &                                                   &                                            &                                                              & \attackMitigatedMark {\tiny \cite{kariyappa_defending_2020}}               & \attackMitigatedMark {\tiny \cite{orekondy_prediction_2020}}                   &                                                 &                                                                   \\ \hline
SMA-\tiny{CNN (PD, AL)}  \tiny{\cite{pal_framework_2019}} &                                                                                                     & \attackMitigatedMark {\tiny \cite{pal_framework_2019}} \speculatemark & \defenceBrokenMark {\tiny \cite{pal_framework_2019}} \speculatemark & \defenceBrokenMark {\tiny \cite{pal_framework_2019}} \speculatemark            &                                                                      &                                                                       &                                                   &                                            & \attackLoweredMark {\tiny \cite{pal_framework_2019}} \speculatemark &                                                              &                                                                  &                                                 &                                                                   \\ \hline
SMA-\tiny{CNN (DS)} \tiny{\cite{mosafi_stealing_2019}}                                              &                                                                                                     &                                                         &                                                         &                                                                    &                                                                      &                                                                       &                                                   &                                            & \defenceBrokenMark {\tiny \cite{mosafi_stealing_2019}} \attackClaimMark        &                                                              &                                                                  &                                                 &                                                                   \\ \hline
SMA-\tiny{CNN (DS)} \tiny{\cite{yuan_es_2022}}                                                      & \defenceBrokenMark {\tiny \cite{yuan_es_2022}}                                                                  &                                                         & \defenceBrokenMark {\tiny \cite{yuan_es_2022}}                      &                                                                    &                                                                      &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  &                                                 &                                                                   \\ \hline
SMA-\tiny{CNN;RNN (Activethief)} \tiny{\cite{pal_activethief_2020}}                                 &                                                                                                     & \defenceBrokenMark {\tiny \cite{pal_activethief_2020}} \attackClaimMark   & \defenceBrokenMark {\tiny \cite{pal_activethief_2020}}              &                                                                    &                                                                      &                                                                       &                                                   &                                            & \defenceBrokenMark {\tiny \cite{pal_activethief_2020}} \attackClaimMark        &                                                              &                                                                  &                                                 &                                                                   \\ \hline
SMA-\tiny{CNN} \tiny{\cite{juuti_prada_2019}}                                                       & \defenceBrokenMark {\tiny \cite{juuti_prada_2019}}                                                              &                                                         & \defenceBrokenMark {\tiny \cite{juuti_prada_2019}}                  &                                                                    &                                                                      &                                                                       & \attackMitigatedMark {\tiny \cite{szyller_dawn_2021}}           &                                            &                                                              &                                                              & \attackMitigatedMark {\tiny \cite{orekondy_prediction_2020}}                   &                                                 &                                                                   \\ \hline
SMA-\tiny{CNN (Knockoff)} \tiny{\cite{orekondy_knockoff_2019}}                                      & \attackLoweredMark {\tiny \cite{orekondy_knockoff_2019}}  \attackMitigatedMark {\tiny \cite{atli_extraction_2020}}       &                                                         &                                                         &                                                                    &                                                                      & \attackMitigatedMark {\tiny \cite{atli_extraction_2020}}                            & \attackMitigatedMark {\tiny \cite{szyller_dawn_2021}}           &                                            &                                                              & \attackMitigatedMark {\tiny \cite{kariyappa_defending_2020}}               &                                                                  &                                                 &                                                                   \\ \hline
SMA-\tiny{CNN} \tiny{\cite{kariyappa_maze_2021}}                                                    & \attackMitigatedMark {\tiny \cite{kariyappa_maze_2021}} \attackClaimMark                                                &                                                         &                                                         &                                                                    &                                                                      &                                                                       &                                                   &                                            & \attackMitigatedMark {\tiny \cite{kariyappa_maze_2021}} \attackClaimMark         & \attackMitigatedMark {\tiny \cite{kariyappa_maze_2021}} \attackClaimMark         & \attackMitigatedMark {\tiny \cite{kariyappa_maze_2021}} \attackClaimMark             &                                                 &                                                                   \\ \hline
SMA-\tiny{CNN (on gradients)} \tiny{\cite{milli_model_2019}}                                        &                                                                                                     &                                                         &                                                         &                                                                    & \attackMitigatedMark {\tiny \cite{chabanne_protection_2020}} \attackClaimMark            &                                                                       &                                                   &                                            &                                                              &                                                              &                                                                  &                                                 &                                                                   \\ \hline
SMA-\tiny{RNN (rand. Quer.} \tiny{\cite{krishna_thieves_2020}}                                      & \defenceBrokenMark {\tiny \cite{krishna_thieves_2020}}                                                          &                                                         &                                                         &                                                                    &                                                                      &                                                                       & \attackMitigatedMark {\tiny \cite{krishna_thieves_2020}}        &                                            &                                                              &                                                              &                                                                  &                                                 &                                                                   \\ \hline
\end{tabular}

}

